Robust Routing and Scheduling of Home Healthcare Workers: A Nested Branch-and-Price Approach

The global home healthcare market is growing rapidly due to aging populations, advancements in healthcare technology, and patient preference for home-based care. In this paper, we study the multi-day planning problem of simultaneously deciding patient acceptance, assignment, routing, and scheduling under uncertain travel and service times. Our approach ensures cardinality-constrained robustness with respect to timely patient care and the prevention of overtime. We take into account a wide range of criteria including patient time windows, caregiver availability and compatibility, a minimum time interval between two visits of a patient, the total number of required visits, continuity of care, and profit. We use a novel systematic modeling scheme that prioritizes health-related criteria as hard constraints and optimizes cost and preference-related criteria as part of the objective function. We present a mixed-integer linear program formulation, along with a nested branch-and-price technique. Results from a case study in Austin, Texas demonstrate that instances of realistic size can be solved to optimality within reasonable runtimes. The price of robustness primarily results from reduced patient load per caregiver. Interestingly, the criterion of geographical proximity appears to be of secondary priority when selecting new patients and assigning them to caregivers.

==> sections/old.tex <==
\label{conclusion}
%\textcolor{gray}{Note: The objective function can be easily changed to not maximize revenue but, e.g., preference satisfaction. Future work may consider accepting patients on a rolling horizon, and including breaks.}

%It's an important consideration to look at patients with visits with different caregivers in the same planning horizon, ensuring that the visits do not overlap. Many of the patients had this issue. 
%Different services: It can of course be solved lexicographically w.r.t. the most expensive jobs, and adjusting the time windows of patients. However, it would be interesting, even though considerably difficult, to find optimal solutions with according constraints.

This work introduces a comprehensive decision tool for patient selection, caregiver assignment, and multi-day routing and scheduling, taking into account polyhedral uncertainty sets for travel and service times. It incorporates a variety of optimization criteria, including patient time windows, number of required visits, caregiver availability, compatibility, continuity of care, and profit. The tool is designed to ensure optimal treatment for all selected patients, considering the factors influenced by operational planning. In particular, all plans are robust, ensuring timely availability for patients and caregivers even in worst-case scenarios, which can be adjusted through uncertainty budgets. At the same time, profit is maximized, calculated as revenue minus wage cost and travel~cost. 


We efficiently decompose the robust home healthcare routing and scheduling problem in several layers for a nested branch-and-price procedure. In the first layer, the problem is decomposed by caregiver, yielding weekly plans. Next, the problem of finding a weekly plan for each caregiver is decomposed by day, yielding daily routes for each. 
These  routes are computed using a branch-and-bound procedure, with traveling salesman subproblems (R-TSPTW), and a multi-knapsack problem guiding the acceptance decision.

%We use the first two layers of this decomposition within a branch-and-price framework. %The advantage is that we actually consider travel cost also in the objective function.

%Daily route determination is addressed using a branch-and-bound method, with a Knapsack problem guiding acceptance decisions and traveling salesman subproblems (R-TSPTW).


Our case study with real data from a large US home healthcare agency demonstrates that, while runtimes increase with shorter time windows and the level of robustness, all instances can be optimally solved within reasonable computation times. Surprisingly, geographic factors seem secondary to revenue and feasibility in the acceptance and assignment of new patients. Compared to parameter settings absent of robustness and time windows, introducing a medium level of robustness and one-hour time windows, and thus smoother operations and a higher service level, leads to an average profit loss of 14.20\%. This is mainly due to decreased patient loads per caregiver per day. 
Nevertheless, some daily schedules can be robustified by scheduling more buffer times without affecting revenue.

%Moreover, there is a trade-off between good service for existing patients (robustness and tight time windiws) on the one hand and health access and possibly fairness on the other hand.

%Limitations: Independency of caregivers ... We point to potentials in the branch-and-price framework, which is that we do not use parallelization, keep all columns, and do not use the gap as suggested in xx. Data specificity. 

Our work also points to several directions for future research. Firstly, the problem setting could be expanded. Alternative objectives such as preference satisfaction and workload balance, additional constraints for lunch breaks, caregiver dependencies, as well as uncertain caregiver absence are also relevant from a practical standpoint.
Secondly, runtimes could be further accelerated. While we solved the R-TSPTW subproblems using Gurobi, it seems promising, particularly for settings with high uncertainty, to employ a problem-specific solution method.
Thirdly, it is intriguing to investigate optimal acceptance and assignment policies. This could include a comparison of our approach with advanced clustering approaches. We also need more research on fair acceptance procedures for new patients.

% Moreover, it would be interesting to add lunch break constraints and to consider different types of visits. Moreover, it would be interesting to integrate dependencies between caregivers and investigate the effect on the nested branch-and-price procedure. After consultation with practitioners, it would be interesting to integrate caregiver's no-shows into our robust framework. Second, runtimes could be accelerated: We solve the R-TSPTW using Gurobi, and it would be promising and in particular for high uncertainties, relevant to accelerate the solution.  Third, it would be interesting to study optimal or approximately optimal acceptance and assignment policies, in particular also comparing the current one to an advanved clustering method. Moreover, more research should be done on fair acceptance policies of new patients. 


